Risk-Bounded Temporal Logic Control of Continuous-Time Stochastic Systems

Motivated by the recent interest in risk-aware control, we study a continuous-time control synthesis problem to bound the risk that a stochastic linear system violates a given specification. We use risk signal temporal logic as a specification formalism in which distributionally robust risk predicates are considered and equipped with the usual Boolean and temporal operators. Our control approach relies on reformulating these risk predicates as deterministic predicates over mean and covariance states of the system. We then obtain a timed sequence of sets of mean and covariance states from the timed automata representation of the specification. To avoid an explosion in the number of automata states, we propose heuristics to find candidate sequences effectively. To execute and check dynamic feasibility of these sequences, we present a sampled-data control technique based on time discretization and constraint tightening that allows to perform timed transitions while satisfying the continuous-time constraints.

==> sections/background.tex <==




\section{Preliminaries and Problem Formulation}

Main contribution: The way I see it right now, we would have the same risk-based STL fragment. However, we may be able or think to obtain guarantees for continuous time (and not only discrete-time). This would be the more theoretical part. The second contribution is based on our observation that the MILPs seemingly fail quickly. Here we can do the automaton offline, and only have to solve smaller MILPs (or whichever control method we use) online. Did I miss anything?

Outline:
\begin{itemize}
    \item Use same risk-based STL fragment \textit{\textbf{(do we need this?)}}
    \item \textbf{Find continuous-time guarantees}
    \item Form automaton offline
    \begin{itemize}
        \item \textbf{Account for \textit{some risk} while using [O1-2]}
        \item \textbf{Modify [O3-5] to account with system uncertainty}
    \end{itemize}
    \item Solve small MILPs online in a similar way to our previous paper (this might be deterministic since we already accounted for risk before) (we can also use CBFs or something else)
\end{itemize}

\subsection{Risk-based Signal Temporal Logic}
In \cite{safaoui2020control} we have STL with a risk operator. Since SITL is a fragment of STL, the same risk formulation applies to it.

In \cite{lindemann2020efficient} SITL to MITL conversion through the $Pr$ operator which replaces predicates by propositions and vice versa.


\subsection{From MITL to Timed Signal Transducer}
\label{sec:mitl_to_ta}

\begin{figure*}
	\centering
	\begin{subfigure}{0.48\textwidth}
		\centering
		\includegraphics[scale=0.265]{figures/until}\caption{Timed signal transducer for $U_{(0,\infty)}$}\label{fig:until}
	\end{subfigure}
	\begin{subfigure}{0.48\textwidth}
		\centering
		\includegraphics[scale=0.265]{figures/eventually}\caption{Timed signal transducer for $F_{(0,b)}$}\label{fig:eventually}
	\end{subfigure}\\
	\begin{subfigure}{0.48\textwidth}
		\centering
		\includegraphics[scale=0.265]{figures/negation}\caption{Timed signal transducer for $\neg$}\label{fig:neg}
	\end{subfigure}
	\begin{subfigure}{0.48\textwidth}
		\centering
		\includegraphics[scale=0.265]{figures/conjunction}\caption{Timed signal transducer for $\wedge$}\label{fig:conjunction}
	\end{subfigure}\\
	\begin{subfigure}{0.48\textwidth}
		\centering
		\includegraphics[scale=0.3]{figures/formula_tree}\caption{Formula tree for  $\varphi:=G_{(0,\infty)}F_{[0,5)} \neg p_1 \vee (p_2 U_{[0,10]} p_3 \wedge G_{(0,15)}p_4)$.}\label{fig:formula_tree}
	\end{subfigure}
	\caption{Displayed are timed signal transducers for Boolean and temporal operators as well as an example of a formula tree. Note that the variables $d$, $d_1$, and $d_2$ in Figs. \ref{fig:until}-\ref{fig:conjunction} are used here as generic input symbols for any inputs according to the formula tree, while $y$ is a generic  output symbol.}
	\label{fig:tsd_temporal}
\end{figure*}


Instead of predicates and uncontrollable propositions, metric interval temporal logic (MITL) considers (controllable) propositions $p\in P$  where $P$ is a set of propositions. An MITL formula $\varphi$ is  an ReRiSITL formula only over propositions \cite{alur1996benefits}. The MITL syntax is hence
\begin{align}\label{eq:full_MITL}
\varphi \; ::= \; \top \; | \; p \; | \;  \neg \varphi \; | \; \varphi' \wedge \varphi'' \; | \; \varphi'  U_I \varphi''\;
\end{align}
where $\varphi'$ and $\varphi''$ are MITL formulas. Let $\boldsymbol{d}:\mathbb{R}_{\ge 0}\to \mathbb{B}^{|P|}$ be a Boolean signal corresponding to truth values of the propositions in $P$ over time. Define again the projection of $\boldsymbol{d}$ onto  $p\in P$ as proj$_p(\boldsymbol{d}):\mathbb{R}_{\ge 0}\to \mathbb{B}$. Given $P$, the expression $(\boldsymbol{d},P,t)\models \varphi$ indicates that the signal $\boldsymbol{d}$ satisfies an MITL formula $\varphi$ at time $t$. The continuous-time semantics of an MITL formula \cite[Sec. 4]{ferrere2019real} are then defined as $(\boldsymbol{d},P,t)\models p$ iff proj$_p(\boldsymbol{d})(t)=\top$, $(\boldsymbol{d},P,t)\models \neg \varphi$ iff $(\boldsymbol{d},P,t)\not\models \varphi$, $(\boldsymbol{d},P,t)\models \varphi'\wedge\varphi''$ iff $(\boldsymbol{d},P,t)\models \varphi'$ and $(\boldsymbol{d},P,t)\models \varphi''$, and $(\boldsymbol{d},P,t)\models \varphi'U_I\varphi''$ iff $\exists t'' \in t\oplus I$, $(\boldsymbol{d},P,t'')\models \varphi''$ and $\forall t' \in (t,t'')$, $(\boldsymbol{d},P,t')\models \varphi'$. An MITL formula $\varphi$ is satisfiable if $\exists \boldsymbol{d}\in \mathcal{F}(\mathbb{R}_{\ge 0},\mathbb{B})$ such that $(\boldsymbol{d},P,0)\models\varphi$. Note that the symbols $\varphi$ and $\phi$ are used to distinguish between MITL and ReRiSITL formulas, respectively. 


An MITL formula $\varphi$ can be translated into a language equivalent timed signal transducer \cite{ferrere2019real} by means of a simple compositional procedure, as summarized next.  Let $\boldsymbol{c}:=\begin{bmatrix} c_1 &\hdots &c_O \end{bmatrix}^T\in\mathbb{R}_{\ge 0}^O$ be a vector of $O$ clock variables that obey the continuous dynamics $\dot{c}_o(t):=1$ with $c_o(0):=0$ for $o\in\{1,\hdots,O\}$. Discrete dynamics occur at instantaneous times in form of clock resets. Let $r:\mathbb{R}_{\ge 0}^O\to \mathbb{R}_{\ge 0}^O$ be a reset function such that $r(\boldsymbol{c})=\boldsymbol{c}'$ where either $c_o'=c_o$ or $c_o'=0$. With a slight abuse of notation, we use $r(c_o)=c_o$ and $r(c_0)=0$. Clocks evolve with time when visiting a state of a timed signal transducer, while clocks may be reset during transitions between states. We define clock constraints as Boolean combinations of conditions of the form $c_o\le k$ and $c_o\ge k$ for some $k\in\mathbb{Q}_{\ge 0}$. Let $\Phi(\boldsymbol{c})$ denote the set of all clock constraints over clock variables in $\boldsymbol{c}$. 
\begin{definition}[Timed Signal Transducer \cite{ferrere2019real}]
	A timed signal transducer is a tuple $TST:=(S,s_0,\Lambda,\Gamma,\boldsymbol{c},\iota,\Delta,\lambda,\gamma, \mathcal{A})$ where $S$ is a finite set of locations, $s_0$ with $s_0\cap S=\emptyset$ is the initial state, $\Lambda$ and $\Gamma$ are a finite sets of input and output variables, respectively, $\iota:S\to\Phi(\boldsymbol{c})$ assigns clock constraints over $\boldsymbol{c}$ to each location, $\Delta$ is a transition relation so that $\delta=(s,g,r,s')\in\Delta$ indicates a transition from $s\in S\cup s_0$ to $s'\in S$ satisfying the guard constraint $g\subseteq \Phi(\boldsymbol{c})$ and resetting the clocks according to $r$; $\lambda:S\cup\Delta\to BC(\Lambda)$ and $\gamma:S\cup\Delta\to BC(\Gamma)$ are input and output labeling functions where $BC(\Lambda)$ and $BC(\Gamma)$ denote the sets of all Boolean combinations over $\Lambda$ and $\Gamma$, respectively, and $\mathcal{A}\subseteq 2^{S\cup \Delta}$ is a generalized B\"uchi acceptance condition.
\end{definition} 



A run of a $TST$ over an input signal $\boldsymbol{d}:\mathbb{R}_{\ge 0}\to \mathbb{B}^{|\Lambda|}$ is an alternation of time and discrete steps resulting in an output signal $\boldsymbol{y}:\mathbb{R}_{\ge 0}\to \mathbb{B}^{|\Gamma|}$. A time step of duration $\tau\in\mathbb{R}_{>0}$ is denoted by $(s,\boldsymbol{c}(t))\xrightarrow{\tau}(s,\boldsymbol{c}(t)+\tau)$ with $\boldsymbol{d}(t+t')\models\lambda(s)$, $\boldsymbol{y}(t+t')\models\gamma(s)$, and $\boldsymbol{c}(t+t')\models \iota(s)$ for each $t'\in (0,\tau)$. A discrete step at time $t$ is denoted by $(s,\boldsymbol{c}(t))\xrightarrow{\delta}(s',r(\boldsymbol{c}(t)))$ for some transition $\delta=(s,g,r,s')\in\Delta$ such that $\boldsymbol{d}(t)\models\lambda(\delta)$, $\boldsymbol{y}(t)\models\gamma(\delta)$, and $\boldsymbol{c}(t)\models g$. Each run starts with a disrete step from the initial configuration $(s_0,\boldsymbol{c}(0))$. Formally, a run of a $TST$ over $\boldsymbol{d}$ is a sequence $(s_0,\boldsymbol{c}(0))\xrightarrow{\delta_0}(s_1,r_0(\boldsymbol{c}(0)))\xrightarrow{\tau_1}(s_1,r_0(\boldsymbol{c}(0))+\tau_1)\xrightarrow{\delta_1} \hdots$. Due to the alternation of time and disrete steps, the signals $\boldsymbol{d}(t)$ and $\boldsymbol{y}(t)$ may be a concatenation of sequences consisting of points and open intervals. Zeno signals are excluded by assumption \cite{ferrere2019real}. We associate a function $q:\mathbb{R}_{\ge 0}\to S\cup \Delta$ with a run as $q(0):=\delta_0$, $q(t)=s_1$ for all $t\in(0,\tau_1)$, $\hdots$; $\mathcal{A}$ is a generalized B\"uchi acceptance condition so that a run over $\boldsymbol{d}(t)$ is accepting if, for each $F\in\mathcal{A}$, $\text{inf}(q)\cap F\neq \emptyset$ where $\text{inf}(q)$ contains the states in $S$ that are visited, in $q$, for an unbounded time duration and transitions in $\Delta$  that are taken, in $q$, infinitely many times. We define the language of $TST$ to be $L(TST):=\{\boldsymbol{d}:\mathbb{R}_{\ge 0}\to \mathbb{R}^{|\Lambda|}|TST\text{ has an accepting run over } \boldsymbol{d}(t)\}$. 
\begin{definition}[Synchronous Product \cite{ferrere2019real}]\label{def:synch_prodd}
	Given $TST_i:=(S_i,s_{0,i},\Lambda_i,\Gamma_i,\boldsymbol{c}_i,\iota_i,\Delta_i,\lambda_i,\gamma_i, \mathcal{A}_i)$ with $i\in\{1,2\}$, their synchronous product is  $TST:=(S,s_0,\Lambda,\Gamma,\boldsymbol{c},\iota,\Delta,\lambda,\gamma, \mathcal{A})$ with $S:=S_1 \times S_2$, $s_0:=s_{0,1}\times s_{0,2}$, $\Lambda:=\Lambda_1\cup \Lambda_2$, $\Gamma:=\Gamma_1\cup \Gamma_2$, $\boldsymbol{c}:=\begin{bmatrix}\boldsymbol{c}_1^T & \boldsymbol{c}_2^T \end{bmatrix}^T$, and  $\iota(s_1,s_2):=\iota_1(s_1)\wedge \iota(s_2)$. The transition relation $\Delta$ is defined as
	\begin{itemize}
		\item $((s_1,s_2),g,r,(s_1',s_2'))\in\Delta$ where $(s_1,g_1,r_1,s_1')\in\Delta_1$, $(s_2,g_2,r_2,s_2')\in\Delta_2$, $g:=g_1\wedge g_2$, and $r:=\begin{bmatrix}r_1^T & r_2^T\end{bmatrix}^T$ (simultaneous transitions),
		\item $((s_1,s_2),g_1 \wedge \iota_2(s_2),r_1,(s_1',s_2))\in\Delta$ where $(s_1,g_1,r_1,s_1')\in\Delta_1$ (left-sided transitions),
		\item $((s_1,s_2),\iota_1(s_1)\wedge g_2,r_2,(s_1,s_2'))\in\Delta$ where $(s_2,g_2,r_2,s_2')\in\Delta_2$ (right-sided transitions),
	\end{itemize}
	and the input labeling function defined as
	\begin{itemize}
		\item $\lambda(s_1,s_2):=\lambda_1(s_1)\wedge \lambda_2(s_2)$ (state labels),
		\item $\lambda((s_1,s_2),g,r,(s_1',s_2')):=\lambda_1(s_1,g_1,r_1,s_1')\wedge \lambda_2(s_2,g_2,r_2,s_2')$ (simultaneous transitions), 
		\item $\lambda((s_1,s_2),g_1\wedge\iota_2(s_2),r_1,(s_1',s_2)):=\lambda_1(s_1,g_1,r_1,s_1')\wedge\lambda_2(s_2)$ (left-sided transitions), 
		\item $\lambda((s_1,s_2),\iota_1(s_1)\wedge g_2,r_2,(s_1,s_2')):=\lambda_1(s_1)\wedge\lambda_2(s_2,g_2,r_2,s_2')$ (right-sided transitions)
	\end{itemize}
	while the output labeling function is constructed the same way as the input labeling function. The B\"uchi acceptance condition is $\mathcal{A}:=\{\mathcal{A}_1\times (S_2\cup \Delta_2), (S_1\cup\Delta_1)\times \mathcal{A}_2\}$.
\end{definition}
\begin{definition}[Input-Output Composition \cite{ferrere2019real}]\label{def:i-o-comp}
	Given $TST_i:=(S_i,s_{0,i},\Lambda_i,\Gamma_i,\boldsymbol{c}_i,\iota_i,\Delta_i,\lambda_i,\gamma_i, \mathcal{A}_i)$ with $i\in\{1,2\}$, the input-output composition where the output of $TST_1$ is the input of $TST_2$ is $TST:=(S,s_0,\Lambda,\Gamma,\boldsymbol{c},\iota,\Delta,\lambda,\gamma, \mathcal{A})$ with $S:=\{(s_1,s_2)\in S_1 \times S_2|\text{if } \boldsymbol{d}\models \gamma_1(s_1)\text{ implies } \boldsymbol{d}\models\lambda_2(s_2)\}$, $\Lambda:=\Lambda_1$, $\Gamma:= \Gamma_2$, and $s_0$, $\boldsymbol{c}$, $\iota$, and $\mathcal{A}$ as defined in the synchronous product. The transition relation $\Delta$ is defined as
	\begin{itemize}
		\item $((s_1,s_2),g,r,(s_1',s_2'))\in\Delta$ where $\delta_1:=(s_1,g_1,r_1,s_1')\in\Delta_1$, $\delta_2:=(s_2,g_2,r_2,s_2')\in\Delta_2$, $g=g_1\wedge g_2$, and $r:=\begin{bmatrix}r_1^T & r_2^T\end{bmatrix}^T$ if $\boldsymbol{d}\models \gamma_1(\delta_1)$ implies $\boldsymbol{d}\models\lambda_2(\delta_2)$ (simultaneous transitions),
		\item $((s_1,s_2),g_1 \wedge \iota_2(s_2),r_1,(s_1',s_2))\in\Delta$ where $\delta_1:=(s_1,g_1,r_1,s_1')\in\Delta_1$ if $\boldsymbol{d}\models \gamma_1(\delta_1)$ implies $\boldsymbol{d}\models\lambda_2(s_2)$ (left-sided transitions),
		\item $((s_1,s_2),\iota_1(s_1)\wedge g_2,r_2,(s_1,s_2'))\in\Delta$ where $\delta_2:=(s_2,g_2,r_2,s_2')\in\Delta_2$ if $\boldsymbol{d}\models\gamma_1(s_1)$ implies $\boldsymbol{d}\models\lambda_2(\delta_2)$ (right-sided transitions),
	\end{itemize}
	and the input and output labeling functions are defined as
	\begin{itemize}
		\item $\lambda(s_1,s_2):=\lambda_1(s_1)$ and $\gamma(s_1,s_2):=\gamma_2(s_2)$ (state labels),
		\item  $\lambda((s_1,s_2),g,r,(s_1',s_2')):=\lambda_1(s_1,g_1,r_1,s_1')$ and $\gamma((s_1,s_2),g,r,(s_1',s_2')):=\gamma_2(s_2,g_2,r_2,s_2')$ (simultaneous transitions),
		\item  $\lambda((s_1,s_2),g_1\wedge\iota_2(s_2),r_1,(s_1',s_2)):=\lambda_1(s_1,g_1,r_1,s_1')$ and $\gamma((s_1,s_2),g_1\wedge\iota_2(s_2),r_1,(s_1',s_2)):=\gamma_2(s_2)$ (left-sided transitions),
		\item $\lambda((s_1,s_2),\iota_1(s_1)\wedge g_2,r_2,(s_1,s_2')):=\lambda_1(s_1)$ and $\gamma((s_1,s_2),\iota_1(s_1)\wedge g_2,r_2,(s_1,s_2')):=\gamma_2(s_2,g_2,r_2,s_2')$ (right-sided transitions).
	\end{itemize}
\end{definition}



We can now summarize the procedure of \cite{ferrere2019real}. First, it shown that every MITL formula $\varphi$ can be rewritten using only temporal operators $U_{(0,\infty)}$ and $F_{(0,b)}$ for rational constants $b$ \cite[Lemmas 4.1 and 4.3]{ferrere2019real}. Second, timed signal transducers for $U_{(0,\infty)}$ and $F_{(0,b)}$ are proposed, see Figs. \ref{fig:until} and \ref{fig:eventually} \cite[Figs. 7 and 11]{ferrere2019real}. Note that all states and transitions except for the state indicated by the dashed line in $U_{(0,\infty)}$ are included in  $\mathcal{A}$. We here further propose timed signal transducers for negations and conjunctions, which are only implicitly mentioned in the proof of \cite[Thm. 6.7]{ferrere2019real}, in Figs. \ref{fig:neg} and \ref{fig:conjunction}. Third, the formula tree of an MITL formula $\varphi$ is constructed as illustrated in Fig. \ref{fig:formula_tree}. Each box in the formula tree represents a timed signal transducer. Boxes not consisting of $\neg$, $\wedge$, $U_{(0,\infty)}$, and $F_{(0,b)}$ can again be rewritten with the results from the first step, i.e., they can be written as a combination of $\neg$, $\wedge$, $U_{(0,\infty)}$, and $F_{(0,b)}$. Fourth, input-output composition and the synchronous product are used to obtain a timed signal transducer $TST_\varphi:=(S,s_0,\Lambda,\Gamma,\boldsymbol{c},\iota,\Delta,\lambda,\gamma, \mathcal{A})$ that has accepting runs over $\boldsymbol{d}$, i.e., $\boldsymbol{d}\in L(TST_\varphi)$, with $\boldsymbol{y}(0)=\top$ (meaning that $\gamma(\delta_0)=y$) if and only if $(\boldsymbol{d},0)\models\varphi$ \cite[Thm. 6.7]{ferrere2019real}. Note that $TST_\varphi$ may have several inputs, but only one output, i.e.,  $\boldsymbol{y}(t)$ is a scalar.

\subsection{Problem Formulation}
